Statistical effects of the observer's peculiar velocity on source number counts

The velocity of the Sun with respect to the cosmic microwave background (CMB) can be extracted from the CMB dipole, provided its intrinsic dipole is assumed to be small in comparison. This interpretation is consistent, within fairly large error bars, with the measurement of the correlations between neighboring CMB multipoles induced by the velocity of the observer, which effectively breaks isotropy. In contrast, the source number count dipole was reported to privilege a velocity of the observer with an amplitude which is about twice as large as the one extracted from the entirely kinematic interpretation of the CMB dipole, with error bars which indicate a more and more significant tension. In this work, we study the effect of the peculiar velocity of the observer on correlations of nearby multipoles in the source number counts. We provide an unbiased estimator for the kinetic dipole amplitude, which is proportional to the peculiar velocity of the observer and we compute the expected signal to noise ratio. Near future experiments can achieve better than 5$\%$ constraints on the velocity of the Sun with our estimator.

==> macros.tex <==
% Abréviations maths

\newcommand\pos{\ensuremath{\vec{r}}}
\newcommand\ux{\ensuremath{\vec{u}_x}}
\newcommand\uy{\ensuremath{\vec{u}_y}}
\newcommand\uz{\ensuremath{\vec{u}_z}}

\newcommand\ensN{\ensuremath{\mathbb{N}}\xspace}
\newcommand\ensZ{\ensuremath{\mathbb{Z}}\xspace}
\newcommand\ensQ{\ensuremath{\mathbb{Q}}\xspace}
\newcommand\ensR{\ensuremath{\mathbb{R}}\xspace}
\newcommand\ensC{\ensuremath{\mathbb{C}}\xspace}
\newcommand\ensK{\ensuremath{\mathbb{K}}\xspace}

\newcommand\ph{\ensuremath{\varphi}}
\newcommand\eps{\ensuremath{\varepsilon}}

\newcommand{\cc}{\text{c.c.}}
\newcommand{\cst}{\mathrm{cst}}
\newcommand{\sgn}{\mathrm{sgn}}

%\newcommand\define{\overset{\text{déf.}}{=}}
\newcommand\define{\equiv}
\newcommand{\coordequal}{\overset{*}{=}}
\newcommand\alg[1]{\overline{#1}}
%\newcommand\vect[1]{\overrightarrow{#1}}
\newcommand\vect[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{#1}}
\newcommand\cplx[1]{\underline{#1}}
\newcommand\ex[1]{\mathrm{e}^{#1}}
\renewcommand\i{\ensuremath{\mathrm{i}}}
\renewcommand\j{\ensuremath{\mathrm{j}}}
\renewcommand\Re{\ensuremath{\mathrm{Re}}}
\renewcommand\Im{\ensuremath{\mathrm{Im}}}
\newcommand{\Arg}{\ensuremath{\mathrm{Arg}}}
\newcommand\suite[3]{\ensuremath{(#1)_{#2\in{#3}}}}
\newcommand\transpose[1]{#1^{\rm T}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand\colonne[2]{\begin{pmatrix} #1 \\ #2 \end{pmatrix}}
\newcommand\gcolonne[2]{\begin{pmatrix} #1 \\[1mm] #2 \end{pmatrix}}
\newcommand\Ker{\mathrm{Ker}}

\newcommand\e[1]{_{\text{#1}}}
\newcommand\h[1]{^{\text{#1}}}
\newcommand\U[1]{\:\mathrm{#1}}
\newcommand{\micro}{\hbox{\textmu}}

\newcommand{\dd}{\mathrm{d}}
\newcommand{\Dd}{\mathrm{D}}
\newcommand{\pd}[3][]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}
\newcommand{\ddf}[3][]{\frac{\dd^{#1} #2}{\dd {#3}^{#1}}}
\newcommand{\Ddf}[3][]{\frac{\Dd^{#1} #2}{\dd {#3}^{#1}}}

\newcommand{\grad}{\vec{\nabla}}

\renewcommand\lim[2]{\underset{ #1 \rightarrow #2 }{ \mathrm{lim} } \,}
\newcommand\tendvers[2]{\underset{#1 \rightarrow #2}{\longrightarrow}}

\newcommand{\delimiters}[4][]{
\ifthenelse{ \equal{#1}{1} }{  #2 #3 #4  }
					{ \ifthenelse{\equal{#1}{2}}{ \big#2 #3 \big#4 }
						{ \ifthenelse{\equal{#1}{3}}{ \Big#2 #3 \Big#4 }
							{ \ifthenelse{\equal{#1}{4}}{ \bigg#2 #3 \bigg#4 }
								{ \ifthenelse{\equal{#1}{5}}{ \Bigg#2 #3 \Bigg#4 }
									{ \left#2 #3 \right#4 }
								}
							}
						}
					}
													}

\newcommand{\pa}[2][]{\delimiters[#1]{(}{#2}{)}}
\newcommand{\pac}[2][]{\delimiters[#1]{[}{#2}{]}}
\newcommand{\paac}[2][]{\delimiters[#1]{\{}{#2}{\}}}
\newcommand{\abs}[2][]{\delimiters[#1]{|}{#2}{|}}
\newcommand{\ev}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\evaluate}[2][]{\delimiters[#1]{.}{#2}{|}}
\newcommand{\mean}[2][]{\delimiters[#1]{\langle}{#2}{\rangle}}
\newcommand{\ket}[2][]{\delimiters[#1]{|}{#2}{\rangle}}
\newcommand{\bra}[2][]{\delimiters[#1]{\langle}{#2}{|}}

\newcommand{\source}{S}
\newcommand{\obs}{O}

\newcommand{\tidal}{\mathcal{R}}
\newcommand{\jacobi}{\mathcal{D}}
\newcommand{\wronski}{\mathcal{W}}
\newcommand{\amplification}{\mathcal{A}}
\newcommand{\deformation}{\mathcal{S}}
\newcommand{\Ricfoc}{\mathscr{R}}
\newcommand{\Weylfoc}{\mathscr{W}}

\newcommand{\Lie}{\mathcal{L}}
\newcommand{\wl}{\mathscr{L}}

\newcommand{\Hc}{\mathcal{H}}

\newcommand{\nul}[1]{%\hat{#1}
#1}

\newcommand{\zero}{\mat{0}}
\newcommand{\identity}{\mat{1}}


\newenvironment{system}
{ \left\{ \begin{aligned} }
{ \end{aligned} \right. }

\newenvironment{remark}
{

\medskip

\noindent
\hspace{0.05\linewidth}
\vline
\hspace{0.01\linewidth}
\begin{minipage}{0.93\linewidth}
}
{
\end{minipage}

\medskip

}

% Box
\newlength{\boxtitlelength}
\newlength{\halfrulelength}
\newcommand{\boxtitle}[1]{\footnotesize\bf{\:#1\:}}
\newenvironment{abox}[1]
{
\setlength{\halfrulelength}{0.5\linewidth}
\settowidth{\boxtitlelength}{\boxtitle{#1}}
\addtolength{\halfrulelength}{-0.5\boxtitlelength}
\noindent\rule[-1mm+1pt]{1pt}{2mm}\rule[1mm]{\halfrulelength}{1pt}{\boxtitle{#1}}\rule[1mm]{\halfrulelength}{1pt}\rule[-1mm+1pt]{1pt}{2mm}\\}
{\\ \rule[1mm]{1pt}{2mm}\noindent\rule[1mm]{\linewidth-2pt}{1pt}\rule[1mm]{1pt}{2mm}}

% Create a command for sections hidden in the text
\newcommand{\hiddensection}[1]{
\refstepcounter{section}
\phantomsection
\addcontentsline{toc}{section}{\protect\numberline{\thesection}#1}
\markright{\thesection \: #1}
}

% Colors

\definecolor{blue4}{RGB}{0,0,143}
\definecolor{red4}{RGB}{143,0,0}
\definecolor{orange}{RGB}{255,128,0}
\definecolor{darkcyan}{RGB}{0,128,128}
\definecolor{olive}{RGB}{0,128,0}
\definecolor{purple}{RGB}{128,0,128}
\definecolor{cyan2}{RGB}{0,255,255}
\definecolor{fushia}{RGB}{255,0,255}
\definecolor{mygray}{gray}{0.5}
\definecolor{lightgray}{gray}{0.85}

% Journals

\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjl}{ApJL}
\newcommand{\aap}{A{\&}A}
\newcommand{\aaps}{A{\&}AS}
\newcommand{\mnras}{MNRAS}
\newcommand{\aj}{AJ}
\newcommand{\araa}{ARAA}
\newcommand{\pasp}{PASP}
\newcommand{\pasj}{PASJ}
\newcommand{\jcap}{JCAP}
\newcommand{\na}{New Astronomy}
\newcommand{\physrep}{Phys. Rep.}
\newcommand{\prd}{Phys. Rev. D}
\newcommand{\azh}{Astron. Zh.}
\newcommand{\nat}{Nature}
\newcommand{\nar}{New Astronomy Reviews}

